Selective Intervention Planning using Restless Multi-Armed Bandits to Improve Maternal and Child Health Outcomes

India has a maternal mortality ratio of 113 and child mortality ratio of 2830 per 100,000 live births. Lack of access to preventive care information is a major contributing factor for these deaths, especially in low resource households. We partner with ARMMAN, a non-profit based in India employing a call-based information program to disseminate health-related information to pregnant women and women with recent child deliveries. We analyze call records of over 300,000 women registered in the program created by ARMMAN and try to identify women who might not engage with these call programs that are proven to result in positive health outcomes. We built machine learning based models to predict the long term engagement pattern from call logs and beneficiaries' demographic information, and discuss the applicability of this method in the real world through a pilot validation. Through a pilot service quality improvement study, we show that using our model's predictions to make interventions boosts engagement metrics by 61.37%. We then formulate the intervention planning problem as restless multi-armed bandits (RMABs), and present preliminary results using this approach.

==> sections/short-term.tex <==
\section{Short term drop-off prediction}

Tracking women who are likely to disengage for an extended period of time based on their past engagement behavior is very important in mitigating the risk of dropping off. The health care worker can intervene with women who are at risk of dropping off the program by providing reminders in the form of phone calls or by even reaching out to them individually. We, therefore, build models that predict if a woman would not answer any calls for the next two weeks given the call history of past 4 weeks and the demographic information.

\subsection{Problem Formulation}
For each beneficiary registered in the program, we randomly sample call sequences spanning six weeks to build our dataset. The data from the first four weeks are used as input features and data from the final two weeks are used to generate the label. If there are no engagements in the final two week period, we label the data as \texttt{high risk}, else it is labelled as \texttt{low risk}. To generate a batch for one training iteration, we sample these sequences from the call logs dataset. We removed the beneficiaries whose demographic features were not complete or were entered in an incorrect format. Additionally, we computed six features from the call logs: number of past attempts, number of past connections, number of past engagements, days since last attempt, days since last connection and days since last engagement.

\begin{figure}[h]
    \centering
    \includegraphics[width=.95\linewidth]{Images/CoNDiP_and_ReNDiP.png}
    \caption{CoNDiP (left) and ReNDiP (right) Architectures}
    \label{fig:ConDiP1}
\end{figure}

\subsection{Models}
For the baseline, provide a rule-based model: beneficiaries having E2C Ratio less than 0.5 in the first four weeks are assigned as high risk and low risk otherwise. The rule-based model basically predicts the future behaviour based on the beneficiary behaviour in the first four weeks after their registration.

We use random forest model over all demographic and call features. The random forest model consists of 200 trees with maximum depth 30. In order to fully utilize the sequential nature of the call histories, we build two neural networks called \textbf{CoNDiP} (Convolutional Neural Disengagement Predictor) and \textbf{ReNDiP} (Recurrent Neural Disengagement Predictor). 

CoNDiP uses 1D Convolutional \cite{kiranyaz20191d} layers to encode the dynamically sized call history features. Since, over the span of 4 weeks at most 8 calls are made to a beneficiary (at most 2 calls per week), we append call sequences having fewer calls with zeroes and feed it to the 1D convolutional layers. 

In CoNDiP, each convolutional layer has 20 kernels of size 3 and there are two convolutional layer after which we do average pooling as follows. Let $f_{i,j}$ be the value of $i$th feature of $j$th call in the output from the 1D convolutional layers. We do average pooling of these features across time to get features $\hat{f}_{i}=\frac{\sum_{j\in [T] }f_{i,j}}{T}$.

We also encode the static features via two feed forward layers with 50 and 100 neurons. Let $g$ be vector of encoded static features output by the feed forward layer. Then, we concatenate $g$ and $\hat{f}$ and feed it through two feed forward layers each with 100 neurons followed by a final layer to compute the probability of being at risk. After each of the feed-forward layers (except last one), we applied batch normalization. 

We also experiment with encoding time-series data with recurrent layers instead of convolutional layers. By replacing the 1D convolutional layers and average pooling with an LSTM \cite{hochreiter1997long} whose output from the last time-step is taken as input to final feed forward layer, we get \textbf{ReNDiP} (Recurrent Neural Disengagement Predictor). We used a bi-directional LSTM with 100 hidden units. The architectures of CoNDiP and ReNDiP are shown in Figure \ref{fig:ConDiP1}.

\begin{table}[h]
\centering
\caption{Results for Short-term Engagement Task}
\begin{tabular}{|c|c|c|c|c|}
\hline
Model        & Accuracy & Precision & Recall & F1 score \\ \midrule
RF$^{\mathrm{a}}$ & 0.846     & 0.859       & 0.832   & 0.847     \\ \hline
%NN-Static    & 0.75     & 0.64      & 0.89   & 0.75     \\ \hline
CoNDiP       & 0.847     & 0.865      & 0.905   & 0.884     \\ \hline
ReNDiP       & 0.841     & 0.851      & 0.913   & 0.881     \\ \hline
Rule-Based & 0.806 & 0.862 & 0.832 & 0.847 \\ \hline
\multicolumn{5}{l}{$^{\mathrm{a}}$RF: Random Forest}
\end{tabular}
\label{tab:short-term}
\end{table}

\begin{figure}[h]
    \centering
    \includegraphics[width=.8\linewidth]{Images/roc_auc-short.png}
    \caption{ROC curve and area under the curve (in legend) for the models for short-term engagement task}
    \label{fig:short-term}
\end{figure}

\subsection{Results}

The results of our models and baseline are summarized in Table \ref{tab:short-term}. The precision, recall, and F-1 scores are reported over the high risk class only since ARMMAN requires models that work well over the high risk class. For all results in further sections too, we report these metrics for the high risk class. CoNDiP and RF show similar performance scores and clearly outperform the baseline. Due to slightly higher scores, CoNDiP is the model best suited for prediction of short-term program engagement. The ROC curves are shown in Figure \ref{fig:short-term}. AUC scores of CoNDiP and RF are marginally higher than that of ReNDiP.

